Applying Inter-rater Reliability and Agreement in Grounded Theory Studies in Software Engineering

In recent years, the qualitative research on empirical software engineering that applies Grounded Theory is increasing. Grounded Theory (GT) is a technique for developing theory inductively e iteratively from qualitative data based on theoretical sampling, coding, constant comparison, memoing, and saturation, as main characteristics. Large or controversial GT studies may involve multiple researchers in collaborative coding, which requires a kind of rigor and consensus that an individual coder does not. Although many qualitative researchers reject quantitative measures in favor of other qualitative criteria, many others are committed to measuring consensus through Inter-Rater Reliability (IRR) and/or Inter-Rater Agreement (IRA) techniques to develop a shared understanding of the phenomenon being studied. However, there are no specific guidelines about how and when to apply IRR/IRA during the iterative process of GT, so researchers have been using ad hoc methods for years. This paper presents a process for systematically applying IRR/IRA in GT studies that meets the iterative nature of this qualitative research method, which is supported by a previous systematic literature review on applying IRR/RA in GT studies in software engineering. This process allows researchers to incrementally generate a theory while ensuring consensus on the constructs that support it and, thus, improving the rigor of qualitative research. This formalization helps researchers to apply IRR/IRA to GT studies when various raters are involved in coding. Measuring consensus among raters promotes communicability, transparency, reflexivity, replicability, and trustworthiness of the research.

==> tables/DataExtraction.tex <==
\onecolumn
\tiny
\begin{longtable}{|l|l|l|l|l|c|c|c|l|}
\caption{Data extraction}
\hline \textbf{ID} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{c}Epistemology\\ Ontology\end{tabular}}} & \multicolumn{1}{c|}{\textbf{GT variant}} & \multicolumn{1}{c|}{\textbf{Recollection  method}} & \multicolumn{1}{c|}{\textbf{GT Coding Phases}} & \textbf{IRA} & \textbf{IRR} & \textbf{Correctly 			used?} & \multicolumn{1}{c|}{\textbf{Coefficient}} \\ \endhead  \hline
\hline
01   & Not mentioned   & Straussian GT      & Interviews data     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
05   & Not mentioned   & Straussian GT      & Video data   & Not mentioned      & -- & IRR  & No (IRA)   & Fleiss $\kappa$    \\ \hline
07   & Not mentioned   & Straussian GT      & Literature      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Const.\ comparison\end{tabular} & -- & IRR  & No (IRA)   & Krippendorff's $\alpha$      \\ \hline
08   & Not mentioned   & \begin{tabular}[c]{@{}l@{}}Straussian GT\\ (inductive analysis)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Screen recordings \\ Survey data \\ Interviews data\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Affinity diagramming \\ Memoing\end{tabular}      & -- & IRR  & No (IRA)   & Fleiss’s $\kappa$    \\ \hline
11   & Not mentioned   & Inductive analysis   & Twitter data      & Open coding        & -- & IRR  & No (IRA)   & $\kappa$ (unknown version)  \\ \hline
12   & Not mentioned   & Straussian GT      & Interviews data     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$  \\ \hline
13   & Not mentioned   & Not mentioned      & Interviews data     & Axial coding       & IRA  & -- & Yes    & Cohen’s $\kappa$  \\ \hline
17   & Not mentioned   & Not mentioned      & \begin{tabular}[c]{@{}l@{}}Video data\\ Text specifications\end{tabular}    & Not mentioned      & -- & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Percent agreement\\ Cohen’s $\kappa$\end{tabular}     \\ \hline
24   & Not mentioned   & Classic GT    & Discourse files     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & -- & IRR  & No (IRA)   & $\kappa$ (unknown version) \\ \hline
26   & Constructivism     & Straussian GT      & Survey data  &    & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$ \\ \hline
28   & Not mentioned   & Straussian GT      & Survey data  & Open coding        & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$   \\ \hline
31   & Not mentioned   & Not mentioned      & Focus group results      & Not mentioned      & -- & IRR  & Yes  & Not mentioned     \\ \hline
34   & Not mentioned   & Straussian GT      & Interviews data     & Open coding        & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
37   & Not mentioned   & Straussian GT      & Interviews data     & Open coding        & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
41   & Not mentioned   & GT-like approach     & Logs     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Thematic analysis\end{tabular}    & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
44   & Not mentioned   & GT-like approach     & Interview data & Open coding        & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
55   & Not mentioned   & GT-like approach     & Literature      & Not mentioned      & -- & IRR  & Yes  & Kendall’s    \\ \hline
57   & Not mentioned   & GT-like approach     & Interview data      & Inductive analysis      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
58   & Constructivism     & Charmaz GT    & \begin{tabular}[c]{@{}l@{}}Interview data\\ Survey data\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Inductive analysis\\ Memoing\end{tabular}     & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
59   & Not mentioned   & GT-like approach     & Literature data     &    & IRA  & -- &  Yes & Krippendorff’s $\alpha$   \\ \hline
60   & Not mentioned   & Straussian GT      & \begin{tabular}[c]{@{}l@{}}Text specifications \\ (users reviews) \end{tabular}    & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
61   & Not mentioned   & GT-like approach     & Text specifications      &    & IRA  & -- &   & Fleiss’s $\kappa$    \\ \hline
62   & Constructivism     & Straussian GT      & Survey data  & Not mentioned      & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
65   & Not mentioned   & Charmaz GT    & \begin{tabular}[c]{@{}l@{}} Text specifications \\ (functional requirements) \end{tabular} & Not mentioned      & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
66   & Not mentioned   & Straussian GT      & \begin{tabular}[c]{@{}l@{}}Video data\\  Text data (comments)\end{tabular}   & Not mentioned      & IRA  & -- &  Yes & Cohen’s $\kappa$  \\ \hline
67   & Not mentioned   & Straussian GT      & Interview data      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Const.\ comparison\end{tabular} & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
74   & Not mentioned   & GT-like approach     & Interview data      & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
78   & Not mentioned   & GT-like approach     & Interview data      & Content Analysis   & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
83   & Not mentioned   & GT-like approach     & Survey data  & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
87   & Not mentioned   & Charmaz GT    & \begin{tabular}[c]{@{}l@{}}Case studies data: \\ Text specifications \\ and images (diagrams)\end{tabular}  & Memoing        & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
88   & Not mentioned   & Straussian GT      & Survey data  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$    \\ \hline
89   & Not mentioned   & GT-like approach     & Interview data      & \begin{tabular}[c]{@{}l@{}}Content analysis\\ Thematic analysis\end{tabular}      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
92   & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Instagram data      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Const.\ comparison\end{tabular}     & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
97   & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Interview data      & \begin{tabular}[c]{@{}l@{}}Initial coding\\ Open coding\\ Axial Coding\end{tabular}   & -- & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Cohen’s $\kappa$\\ Scott’s $\pi$ \end{tabular} \\ \hline
102  & Not mentioned   & GT-like approach     & \begin{tabular}[c]{@{}l@{}}Logs\\ Text specifications\end{tabular} & \begin{tabular}[c]{@{}l@{}}Initial coding\\ Axial coding\end{tabular}      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
110  & Not mentioned   & GT-like approach     & Audio data   & Not mentioned      & -- & IRR  & No (IRA \& IRR) & \begin{tabular}[c]{@{}l@{}}Cohen’s $\kappa$\\ Shaffer’s $\rho$\end{tabular}     \\ \hline
111  & Not mentioned   & 
     GT-like approach   & \begin{tabular}[l]{@{}l@{}}Interview data\\ Focused group data\end{tabular} & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
128  & Not mentioned   & GT-like approach  & Image data   & Open coding        & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
132  & Not mentioned   & GT-like approach     & Text specifications      & Not mentioned      &   & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Percent agreement\\ Fleiss’ $\kappa$\end{tabular} \\ \hline
138  & Not mentioned   & Straussian-GT    & Text specification  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Content analysis\end{tabular}     & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
140  & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular} & \begin{tabular}[c]{@{}l@{}}Interview data\\ Text specifications\end{tabular}  & Content analysis   & -- & IRR  & No (IRA)   & Kripendorff’s $\alpha$    \\ \hline
144  & Not mentioned   & GT-like approach     & Interview data      & Not specified      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
147  & Not mentioned   & GT-like approach     & Literature data     & Not specified      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
151  & Not mentioned   & GT-like approach     & Text specifications      & Not specified      & -- & IRR  &   & Pearson‘s $r$   \\ \hline
153  & Not mentioned   & Straussian-GT    & Text specifications      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
154  & Not mentioned   & GT-like approach     & Text specifications      & Not specified      & IRA  & -- &   & Fleiss’ $\kappa$     \\ \hline
158  & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Text specifications      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Content analysis\end{tabular}     & -- & IRR  & No (IRA)   & $\kappa$ (unknown version)  \\ \hline
161  & Not mentioned   & GT-like approach     & Interview data      & Not mentioned      & IRA  & -- &   & Percent agreement      \\ \hline
163  & Not mentioned   & GT-like approach     & \begin{tabular}[c]{@{}l@{}}Interviews data\\ Surveys (questionnaires)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline

\label{tab:table6}
\end{longtable}

\twocolumn
\normalsize

==> tables/DataExtraction2.tex <==
\begin{table*}
\centering
\caption{Data extraction}
\label{tab:table6}
\renewcommand{\arraystretch}{1}

\begin{tabular}{|l|l|l|l|l|c|c|c|l|}
\hline \textbf{ID} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{c}Epistemology\\ Ontology\end{tabular}}} & \multicolumn{1}{c|}{\textbf{GT variant}} & \multicolumn{1}{c|}{\textbf{Recollection  method}} & \multicolumn{1}{c|}{\textbf{GT Coding Phases}} & \textbf{IRA} & \textbf{IRR} & \textbf{Correctly 			used?} & \multicolumn{1}{c|}{\textbf{Coefficient}} \\ \endhead  \hline
\hline
01   & Not mentioned   & Straussian GT      & Interviews data     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
05   & Not mentioned   & Straussian GT      & Video data   & Not mentioned      & -- & IRR  & No (IRA)   & Fleiss $\kappa$    \\ \hline
07   & Not mentioned   & Straussian GT      & Literature      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Const.\ comparison\end{tabular} & -- & IRR  & No (IRA)   & Krippendorff's $\alpha$      \\ \hline
08   & Not mentioned   & \begin{tabular}[c]{@{}l@{}}Straussian GT\\ (inductive analysis)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Screen recordings \\ Survey data \\ Interviews data\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Affinity diagramming \\ Memoing\end{tabular}      & -- & IRR  & No (IRA)   & Fleiss’s $\kappa$    \\ \hline
11   & Not mentioned   & Inductive analysis   & Twitter data      & Open coding        & -- & IRR  & No (IRA)   & $\kappa$ (unknown version)  \\ \hline
12   & Not mentioned   & Straussian GT      & Interviews data     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$  \\ \hline
13   & Not mentioned   & Not mentioned      & Interviews data     & Axial coding       & IRA  & -- & Yes    & Cohen’s $\kappa$  \\ \hline
17   & Not mentioned   & Not mentioned      & \begin{tabular}[c]{@{}l@{}}Video data\\ Text specifications\end{tabular}    & Not mentioned      & -- & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Percent agreement\\ Cohen’s $\kappa$\end{tabular}     \\ \hline
24   & Not mentioned   & Classic GT    & Discourse files     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & -- & IRR  & No (IRA)   & $\kappa$ (unknown version) \\ \hline
26   & Constructivism     & Straussian GT      & Survey data  &    & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$ \\ \hline
28   & Not mentioned   & Straussian GT      & Survey data  & Open coding        & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$   \\ \hline
31   & Not mentioned   & Not mentioned      & Focus group results      & Not mentioned      & -- & IRR  & Yes  & Not mentioned     \\ \hline
34   & Not mentioned   & Straussian GT      & Interviews data     & Open coding        & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
37   & Not mentioned   & Straussian GT      & Interviews data     & Open coding        & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
41   & Not mentioned   & GT-like approach     & Logs     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Thematic analysis\end{tabular}    & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
44   & Not mentioned   & GT-like approach     & Interview data & Open coding        & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
55   & Not mentioned   & GT-like approach     & Literature      & Not mentioned      & -- & IRR  & Yes  & Kendall’s    \\ \hline
57   & Not mentioned   & GT-like approach     & Interview data      & Inductive analysis      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
58   & Constructivism     & Charmaz GT    & \begin{tabular}[c]{@{}l@{}}Interview data\\ Survey data\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Inductive analysis\\ Memoing\end{tabular}     & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
59   & Not mentioned   & GT-like approach     & Literature data     &    & IRA  & -- &  Yes & Krippendorff’s $\alpha$   \\ \hline
60   & Not mentioned   & Straussian GT      & \begin{tabular}[c]{@{}l@{}}Text specifications \\ (users reviews) \end{tabular}    & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
61   & Not mentioned   & GT-like approach     & Text specifications      &    & IRA  & -- &   & Fleiss’s $\kappa$    \\ \hline
62   & Constructivism     & Straussian GT      & Survey data  & Not mentioned      & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
65   & Not mentioned   & Charmaz GT    & \begin{tabular}[c]{@{}l@{}} Text specifications \\ (functional requirements) \end{tabular} & Not mentioned      & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
66   & Not mentioned   & Straussian GT      & \begin{tabular}[c]{@{}l@{}}Video data\\  Text data (comments)\end{tabular}   & Not mentioned      & IRA  & -- &  Yes & Cohen’s $\kappa$  \\ \hline
67   & Not mentioned   & Straussian GT      & Interview data      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Const.\ comparison\end{tabular} & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
74   & Not mentioned   & GT-like approach     & Interview data      & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
78   & Not mentioned   & GT-like approach     & Interview data      & Content Analysis   & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
83   & Not mentioned   & GT-like approach     & Survey data  & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
87   & Not mentioned   & Charmaz GT    & \begin{tabular}[c]{@{}l@{}}Case studies data: \\ Text specifications \\ and images (diagrams)\end{tabular}  & Memoing        & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
88   & Not mentioned   & Straussian GT      & Survey data  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$    \\ \hline
89   & Not mentioned   & GT-like approach     & Interview data      & \begin{tabular}[c]{@{}l@{}}Content analysis\\ Thematic analysis\end{tabular}      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
92   & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Instagram data      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Const.\ comparison\end{tabular}     & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
97   & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Interview data      & \begin{tabular}[c]{@{}l@{}}Initial coding\\ Open coding\\ Axial Coding\end{tabular}   & -- & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Cohen’s $\kappa$\\ Scott’s $\pi$ \end{tabular} \\ \hline
102  & Not mentioned   & GT-like approach     & \begin{tabular}[c]{@{}l@{}}Logs\\ Text specifications\end{tabular} & \begin{tabular}[c]{@{}l@{}}Initial coding\\ Axial coding\end{tabular}      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
110  & Not mentioned   & GT-like approach     & Audio data   & Not mentioned      & -- & IRR  & No (IRA \& IRR) & \begin{tabular}[c]{@{}l@{}}Cohen’s $\kappa$\\ Shaffer’s $\rho$\end{tabular}     \\ \hline
111  & Not mentioned   & 
     GT-like approach   & \begin{tabular}[l]{@{}l@{}}Interview data\\ Focused group data\end{tabular} & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
128  & Not mentioned   & GT-like approach  & Image data   & Open coding        & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
132  & Not mentioned   & GT-like approach     & Text specifications      & Not mentioned      &   & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Percent agreement\\ Fleiss’ $\kappa$\end{tabular} \\ \hline
138  & Not mentioned   & Straussian-GT    & Text specification  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Content analysis\end{tabular}     & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
140  & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular} & \begin{tabular}[c]{@{}l@{}}Interview data\\ Text specifications\end{tabular}  & Content analysis   & -- & IRR  & No (IRA)   & Kripendorff’s $\alpha$    \\ \hline
144  & Not mentioned   & GT-like approach     & Interview data      & Not specified      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
147  & Not mentioned   & GT-like approach     & Literature data     & Not specified      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
151  & Not mentioned   & GT-like approach     & Text specifications      & Not specified      & -- & IRR  &   & Pearson‘s $r$   \\ \hline
153  & Not mentioned   & Straussian-GT    & Text specifications      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
154  & Not mentioned   & GT-like approach     & Text specifications      & Not specified      & IRA  & -- &   & Fleiss’ $\kappa$     \\ \hline
158  & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Text specifications      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Content analysis\end{tabular}     & -- & IRR  & No (IRA)   & $\kappa$ (unknown version)  \\ \hline
161  & Not mentioned   & GT-like approach     & Interview data      & Not mentioned      & IRA  & -- &   & Percent agreement      \\ \hline
163  & Not mentioned   & GT-like approach     & \begin{tabular}[c]{@{}l@{}}Interviews data\\ Surveys (questionnaires)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
\end{tabular}
\end{table*}


==> tables/DataExtraction3.tex <==
\begin{table*}
\onecolumn
\tiny
\begin{tabular}{|l|l|l|l|l|c|c|c|l|}
\hline \textbf{ID} & \multicolumn{1}{c|}{\textbf{\begin{tabular}{c}Epistemology\\ Ontology\end{tabular}}} & \multicolumn{1}{c|}{\textbf{GT variant}} & \multicolumn{1}{c|}{\textbf{Recollection  method}} & \multicolumn{1}{c|}{\textbf{GT Coding Phases}} & \textbf{IRA} & \textbf{IRR} & \textbf{\begin{tabular}{c}Correctly \\	used?\end{tabular}} & \multicolumn{1}{c|}{\textbf{Coefficient}} \\   \hline
\hline
01   & Not mentioned   & Straussian GT      & Interviews data     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
05   & Not mentioned   & Straussian GT      & Video data   & Not mentioned      & -- & IRR  & No (IRA)   & Fleiss $\kappa$    \\ \hline
07   & Not mentioned   & Straussian GT      & Literature      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Const.\ comparison\end{tabular} & -- & IRR  & No (IRA)   & Krippendorff's $\alpha$      \\ \hline
08   & Not mentioned   & \begin{tabular}[c]{@{}l@{}}Straussian GT\\ (inductive analysis)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Screen recordings \\ Survey data \\ Interviews data\end{tabular}  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Affinity diagramming \\ Memoing\end{tabular}      & -- & IRR  & No (IRA)   & Fleiss’s $\kappa$    \\ \hline
11   & Not mentioned   & Inductive analysis   & Twitter data      & Open coding        & -- & IRR  & No (IRA)   & $\kappa$ (unknown version)  \\ \hline
12   & Not mentioned   & Straussian GT      & Interviews data     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$  \\ \hline
13   & Not mentioned   & Not mentioned      & Interviews data     & Axial coding       & IRA  & -- & Yes    & Cohen’s $\kappa$  \\ \hline
17   & Not mentioned   & Not mentioned      & \begin{tabular}[c]{@{}l@{}}Video data\\ Text specifications\end{tabular}    & Not mentioned      & -- & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Percent agreement\\ Cohen’s $\kappa$\end{tabular}     \\ \hline
24   & Not mentioned   & Classic GT    & Discourse files     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & -- & IRR  & No (IRA)   & $\kappa$ (unknown version) \\ \hline
26   & Constructivism     & Straussian GT      & Survey data  &    & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$ \\ \hline
28   & Not mentioned   & Straussian GT      & Survey data  & Open coding        & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$   \\ \hline
31   & Not mentioned   & Not mentioned      & Focus group results      & Not mentioned      & -- & IRR  & Yes  & Not mentioned     \\ \hline
34   & Not mentioned   & Straussian GT      & Interviews data     & Open coding        & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
37   & Not mentioned   & Straussian GT      & Interviews data     & Open coding        & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
41   & Not mentioned   & GT-like approach     & Logs     & \begin{tabular}[c]{@{}l@{}}Open coding\\ Thematic analysis\end{tabular}    & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
44   & Not mentioned   & GT-like approach     & Interview data & Open coding        & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
55   & Not mentioned   & GT-like approach     & Literature      & Not mentioned      & -- & IRR  & Yes  & Kendall’s    \\ \hline
57   & Not mentioned   & GT-like approach     & Interview data      & Inductive analysis      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
58   & Constructivism     & Charmaz GT    & \begin{tabular}[c]{@{}l@{}}Interview data\\ Survey data\end{tabular}   & \begin{tabular}[c]{@{}l@{}}Inductive analysis\\ Memoing\end{tabular}     & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
59   & Not mentioned   & GT-like approach     & Literature data     &    & IRA  & -- &  Yes & Krippendorff’s $\alpha$   \\ \hline
60   & Not mentioned   & Straussian GT      & \begin{tabular}[c]{@{}l@{}}Text specifications \\ (users reviews) \end{tabular}    & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
61   & Not mentioned   & GT-like approach     & Text specifications      &    & IRA  & -- &   & Fleiss’s $\kappa$    \\ \hline
62   & Constructivism     & Straussian GT      & Survey data  & Not mentioned      & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
65   & Not mentioned   & Charmaz GT    & \begin{tabular}[c]{@{}l@{}} Text specifications \\ (functional requirements) \end{tabular} & Not mentioned      & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
66   & Not mentioned   & Straussian GT      & \begin{tabular}[c]{@{}l@{}}Video data\\  Text data (comments)\end{tabular}   & Not mentioned      & IRA  & -- &  Yes & Cohen’s $\kappa$  \\ \hline
67   & Not mentioned   & Straussian GT      & Interview data      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Const.\ comparison\end{tabular} & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
74   & Not mentioned   & GT-like approach     & Interview data      & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
78   & Not mentioned   & GT-like approach     & Interview data      & Content Analysis   & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
83   & Not mentioned   & GT-like approach     & Survey data  & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
87   & Not mentioned   & Charmaz GT    & \begin{tabular}[c]{@{}l@{}}Case studies data: \\ Text specifications \\ and images (diagrams)\end{tabular}  & Memoing        & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
88   & Not mentioned   & Straussian GT      & Survey data  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Krippendorff’s $\alpha$    \\ \hline
89   & Not mentioned   & GT-like approach     & Interview data      & \begin{tabular}[c]{@{}l@{}}Content analysis\\ Thematic analysis\end{tabular}      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
92   & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Instagram data      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Const.\ comparison\end{tabular}     & IRA  & -- &  Yes & Cohen’s $\kappa$     \\ \hline
97   & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Interview data      & \begin{tabular}[c]{@{}l@{}}Initial coding\\ Open coding\\ Axial Coding\end{tabular}   & -- & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Cohen’s $\kappa$\\ Scott’s $\pi$ \end{tabular} \\ \hline
102  & Not mentioned   & GT-like approach     & \begin{tabular}[c]{@{}l@{}}Logs\\ Text specifications\end{tabular} & \begin{tabular}[c]{@{}l@{}}Initial coding\\ Axial coding\end{tabular}      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
110  & Not mentioned   & GT-like approach     & Audio data   & Not mentioned      & -- & IRR  & No (IRA \& IRR) & \begin{tabular}[c]{@{}l@{}}Cohen’s $\kappa$\\ Shaffer’s $\rho$\end{tabular}     \\ \hline
111  & Not mentioned   & 
     GT-like approach   & \begin{tabular}[l]{@{}l@{}}Interview data\\ Focused group data\end{tabular} & Not mentioned      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
128  & Not mentioned   & GT-like approach  & Image data   & Open coding        & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
132  & Not mentioned   & GT-like approach     & Text specifications      & Not mentioned      &   & IRR  & No (IRA)   & \begin{tabular}[c]{@{}l@{}}Percent agreement\\ Fleiss’ $\kappa$\end{tabular} \\ \hline
138  & Not mentioned   & Straussian-GT    & Text specification  & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Content analysis\end{tabular}     & IRA  & -- & Yes  & Cohen’s $\kappa$     \\ \hline
140  & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular} & \begin{tabular}[c]{@{}l@{}}Interview data\\ Text specifications\end{tabular}  & Content analysis   & -- & IRR  & No (IRA)   & Kripendorff’s $\alpha$    \\ \hline
144  & Not mentioned   & GT-like approach     & Interview data      & Not specified      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
147  & Not mentioned   & GT-like approach     & Literature data     & Not specified      & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
151  & Not mentioned   & GT-like approach     & Text specifications      & Not specified      & -- & IRR  &   & Pearson‘s $r$   \\ \hline
153  & Not mentioned   & Straussian-GT    & Text specifications      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\end{tabular} & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
154  & Not mentioned   & GT-like approach     & Text specifications      & Not specified      & IRA  & -- &   & Fleiss’ $\kappa$     \\ \hline
158  & Not mentioned   & \begin{tabular}[l]{@{}l@{}}GT but variant\\ is not specified\end{tabular}  & Text specifications      & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\\ Selective coding\\ Content analysis\end{tabular}     & -- & IRR  & No (IRA)   & $\kappa$ (unknown version)  \\ \hline
161  & Not mentioned   & GT-like approach     & Interview data      & Not mentioned      & IRA  & -- &   & Percent agreement      \\ \hline
163  & Not mentioned   & GT-like approach     & \begin{tabular}[c]{@{}l@{}}Interviews data\\ Surveys (questionnaires)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Open coding\\ Axial coding\end{tabular}    & -- & IRR  & No (IRA)   & Cohen’s $\kappa$     \\ \hline
\end{tabular}

\caption{Data extraction}
\label{tab:table6}
\end{table*}

\twocolumn
\normalsize
